Joint Learning of Correlated Sequence Labelling Tasks Using Bidirectional Recurrent Neural Networks

The stream of words produced by Automatic Speech Recognition (ASR) systems is typically devoid of punctuations and formatting. Most natural language processing applications expect segmented and well-formatted texts as input, which is not available in ASR output. This paper proposes a novel technique of jointly modeling multiple correlated tasks such as punctuation and capitalization using bidirectional recurrent neural networks, which leads to improved performance for each of these tasks. This method could be extended for joint modeling of any other correlated sequence labeling tasks.

==> debater.tex <==
\section{Argumentation Mining}
Argumentation Mining is an area in artificial intelligence research which has generated a lot of interest of late. According to \cite{lippi2015}, \textit{Argumentation (or argument) mining involves automatically identifying structured argument data from unstructured natural language corpora, by exploiting the techniques and methods of natural language processing, machine learning, sentiment analysis and computational models of argument.} This field is also known as Computational Argumentation. One of the leading efforts in this direction is the IBM Debater\footnote{https://goo.gl/6c0Npu} project, whose ultimate goal is ``to develop technologies that can assist humans to debate and reason''. This requires understanding the topic of debate and producing supporting or contrasting arguments extracted from generic large-scale textual corpora. 

According to \cite{cdcd2014}, a \textit{claim} is a fundamental concept existing in every argument. A \textit{topic} is ``short phrase that frames the discussion'' in a debate. A \textit{claim-dependent claim}, on the other hand, is ``a general, concise statement that directly supports or contests the given topic''. For example, the following sentence contains a claim, marked in italic, for the motion topic in brackets:

\begin{adjustwidth}{1em}{0pt}
\small
(\textbf{The sale of violent video games to minors should be banned}) Parents fear the \textit{violent video games are influencing their children's view about violence}.\\
%(\textbf{The sale of violent video games to minors should be banned}) Other studies reach the conclusion that \textit{violence in video games is not causally linked with aggressive tendencies}.
\end{adjustwidth}

The italicized claim above is supporting the bolded topic. On the other hand there can be claims (as the one below) which is against the topic:

\begin{adjustwidth}{1em}{0pt}
\small
(\textbf{Gambling should be banned}) \textit{Gambling is also a major international commercial activity}, with the legal gambling market totaling an estimated \$335 billion in 2009.\\
%(\textbf{The sale of violent video games to minors should be banned}) Other studies reach the conclusion that \textit{violence in video games is not causally linked with aggressive tendencies}.
\end{adjustwidth}



==> entailment.tex <==
\subsection{Evaluating on a downstream task} \label{sec:downstream}
The purpose of improving the performance of text normalization tasks such as punctuation and capitalization prediction is ultimately to improve the performance of downstream tasks. In this section we describe assessments of such tasks by comparing the performance of the downstream task on differently processed corpora. The assumption is that the better the corpus is normalized, the best NLP tasks will perform on it.

As the downstream task, we chose Recognizing Textual Entailment (RTE) task, which is used in many NLP applications and for which automatic tools are available. Given a pair of texts termed Text (T) and Hypothesis (H), automatic entailment engines decide whether the meaning of H can be implied from T (denoted T-arrow-H). RTE engines typically rely on parsing and often employ named entity recognition, therefore we expect different preprocessing to have impact on the performance\footnote{We used the open-source BIUTEE entailmet engine (reference), available at URL}. Since there is no labeled TED or IQ2 corpus that we are aware of, we used the dataset from RTE-5 search task (reference). The dataset contains documents and hypotheses, along with annotation which sentences from the documents entail (or do not entail) the hypotheses. We apply RTE task in Information Retrieval setting. Namely, given a hypothesis H we want to retrieve all the documents, which contain at least one sentence T such that T-arrow-H. We remove capitalization and punctuation from the original documents, apply different text normalization models and compare the performance of an RTE engine for the resulting texts. We use a subset of the RTE-5 dataset, with 2 hypotheses per document, resulting in XXXX labeled document-hypothesis pairs.

We compare the following models: (1) Single-BiRNN (punctuation) and (2) Corr-BiRNN.  
Since most of the hypotheses in our dataset contain named entities, we applied the Stanford Truecaser to the output of punct-only model before running the RTE engine. Since joint model adds to the documents both punctuation and capitalization, for fair comparison we evaluate an additional setting: (3) applying the Stanford Truecaser to the lowercased output of the joint model.\footnote{Note that the performance of this truecaser is expected to be somewhat affected by the different punctuations.}

% I want to add how many sentence-hypothesis pairs RTE engine had to annotate for each model. - one more sentence. If it's interesting.

We report the results in terms of micro-averaged Precision (P), Recall (R) and F$_1$.

% table with the results

==> ner.tex <==
\newcommand{\nethreetypes}{3TYPES\xspace}
\newcommand{\neonetype}{1TYPE\xspace}

\subsection{Evaluating on a downstream task} \label{sec:downstream}
The purpose of improving the performance of text normalization tasks such as punctuation and capitalization prediction is ultimately to improve the performance of downstream tasks. In this section we describe assessments of such tasks by comparing the performance of the downstream task on differently processed corpora. The assumption is that the better the corpus is normalized, the best NLP tasks will perform on it.

Since there is no labeled TED or IQ2 corpus that we are aware of, we applied the following assessment procedure: We choose three off-the-shelf tools that can run the same task, apply all of them to the corpus, and count the number of times all three are in consensus over the label. The assumption here is that the better normalization will enable the tools to perform better, which in turn will result in higher consensus. If this assumption is correct, we expect the count on the references to be the highest.  

%use the predictions for which there is majority agreement as the gold standard. Then we apply each of the tools to the corpus, measure its token-level performance relative to the created gold corpus, and average the results. 
%The drawback of this procedure is that is removes the harder cases where the tools don't agree on, thus not accounting for potential improvements from our model on the harder cases.

As the downstream task, we chose Named Entity Recognition (NER), and POS tagging simply due to availability of enough such tools. NER looks at rather local text segments, thus we do not expect punctuation to make a significant difference; we do expect better casing to improve the performance. 
As our three tools, we used the named entity recognizers and part of speech taggers of OpenNLP\footnote{\url{https://opennlp.apache.org}}, Stanford CoreNLP \cite{manning-EtAl:2014:P14-5} and NLTK \cite{bird2006nltk}.
%
We applied the above procedure in each of our three experiments (punctuation-only, case-only and both), comparing the NER results when the corpus is being processed by each of the methods.
%SM 12/3 verify last sentence
%
Since NER performs poorly on lowercased texts, for our punctuation-only experiments, we applied to the text the Stanford Truecaser before running the NER or POS tools. Note that the performance of this truecaser is expected to be somewhat affected by the different punctuations.
%
We assess two NER configurations: the first, where we measure the performance of predicting exactly each of \tc{person}, \tc{location} and \tc{organization} (\nethreetypes{} below), and the second where we collapse the above three entity types into a single 'NE' tag. (\neonetype). 
Table~\ref{tab:ner} shows the results of this experiment in terms of the percentage of consensus labels relative to the reference set.
% SM 12/3 is the above sent clear?

\begin{table}
	\centering
		\begin{tabular}{|c|c|c|c|}
		\hline
		& \nethreetypes (\%) & \neonetype (\%) & POS (\%)\\
		\hline
		Ref. & 140 & 163 & 14576 \\
		\hline
		Single-BiRNN (ASR) & 74.3 & 73.6 & 80.4 \\  %104 & 120 & 11715 \\
		\textbf{Corr-BiRNN} (ASR) & \textbf{77.1} & \textbf{78.5} & \textbf{91.6} \\%\textbf{108} & \textbf{128} & \textbf{13348} \\
		\hline
		\end{tabular} 
		\caption{NER and POS results. For Ref. we show the counts of consensus tags; for the different models, we show the percentage relative to these figures.}\label{tab:ner}
\end{table}

%SM 12/3 still missing: 1) details in the table 2) a conclusion sentence

%We measure micro-average Precision (P), Recall (R) and F$_1$; in the \nethreetypes{} setting we also measure Slot Error Rate (SER) \cite{}, which is equivalent to WER, but considers the tags only and not all tokens.
